Towards A Unified View of Answer Calibration for Multi-Step Reasoning

Large Language Models (LLMs) employing Chain-of-Thought (CoT) prompting have broadened the scope for improving multi-step reasoning capabilities. We generally divide multi-step reasoning into two phases: path generation to generate the reasoning path(s); and answer calibration post-processing the reasoning path(s) to obtain a final answer. However, the existing literature lacks systematic analysis on different answer calibration approaches. In this paper, we summarize the taxonomy of recent answer calibration techniques and break them down into step-level and path-level strategies. We then conduct a thorough evaluation on these strategies from a unified view, systematically scrutinizing step-level and path-level answer calibration across multiple paths. Experimental results reveal that integrating the dominance of both strategies tends to derive optimal outcomes. Our study holds the potential to illuminate key insights for optimizing multi-step reasoning with answer calibration.

==> discussion.tex <==
\iffalse
\bibliography{custom}
\bibliographystyle{acl_natbib}
\fi
% !TEX root = ./arr2024.tex

\section{Discussion}
\label{sec:discussion}

% \subsection{Plan-Then-Acting or Learn-From-Practice?}

\subsection{Prior Planing or Direct Practice?}

TBD

\subsection{Step-Centric or Chain-Centric?} 


==> preliminary.tex <==
\iffalse
\bibliography{custom}
\bibliographystyle{acl_natbib}
\fi
% !TEX root = ./arr2024.tex

\section{Preliminary}
\label{sec:preliminary}


% \capitalisewords
% \textbf{\makefirstuc{\classB}}
\subsection{Formulation of Answer Calibration} 

Given a question denoted as $\mathcal{Q}$ and its associated prompt $\mathcal{P}$, we leverage the LLM to generate the result $\mathcal{R}$. $\mathcal{R}$ can either encompass a single reasoning path $\mathcal{P}$ with an initial answer $A$ or multiple reasoning paths $\mathbb{P} = \{ \mathcal{P}_i \}_{i \in [1, N]}$ with a corresponding answer set $\mathbb{A} = \{ \mathcal{A}_i \}_{i \in [1, N]}$. The total number of paths in $\mathbb{P}$ is $N$. 
In this paper, we analyze under the assumption that each reasoning path comprises a maximum of $M$ steps. Paths with steps exceeding this threshold are truncated, while those with fewer are padded. The intermediate step answers for each reasoning path are represented as $a_t \ (t \in [1, M])$. 
% Reasoning paths exceeding this limit are truncated, while those with fewer steps are padded. 
% contains up to 

\paragraph{Step-level \classB.} 
For a single reasoning path $P$ with an initial final path answer $A$ and intermediate step answers $a_t$, the goal of step-level {\classB} is to rectify any erroneous $a_t$, so that deriving the correct $A$. 
For multiple reasoning paths $\mathbb{P}$, step-level {\classB} seeks to either select the reasoning path with the maximum correct intermediate step answers or aggregate the verified correct steps to form the most accurate reasoning path, leading to a correct final path answer. 
\emph{Self-verification} \cite{EMNLP2023-Findings_Self-Verification} is a classical approach for step-level {\classB} on multiple reasoning paths. 

\paragraph{Path-level \classB.}
For a single reasoning path $P$ with an initial final path answer $A$, the objective of path-level {\classB} is to revise the wrong $A$. 
For multiple reasoning paths $\mathbb{P} = \{ \mathcal{P}_i \}_{i \in [1, N]}$ with corresponding answers $\mathbb{A} = \{ \mathcal{A}_i \}_{i \in [1, N]}$, path-level {\classB} aims to select the reasoning path from $\mathbb{P}$ with the most consistent answer in $\mathbb{A}$. 
\emph{Self-consistency} \cite{ICLR2023_Self-Consistency} stands as a time-honored technique for path-level {\classB} on multiple reasoning paths. 

\paragraph{Proposal: Jointly step-level and path-level {\classB} on multiple paths.} 
Considering the advantages of both step-level and path-level {\classB}, we propose to integrate the two strategies on multiple paths. Given the multiple generated reasoning paths $\mathbb{P} = \{ \mathcal{P}_i \}_{i \in [1, N]}$, we define a score $D_i$ for each $\mathcal{P}_i$ (with the final path answer: $\mathcal{A}_i$ and intermediate step answers: $a_t$): 
\begin{equation}
D_i = \alpha \frac{n_i}{N} + (1 - \alpha) \frac{m_i}{M}
\label{eq:measure_score}
\end{equation}
% \alpha F_i + (1 - \alpha) S_i = 
where $n_i$ is the number of consistent final path answer as $\mathcal{A}_i$ in $\mathbb{A}$, and $m_i$ is the number of correct intermediate steps. 
% Given the context of answer calibration, we aim to establish a mathematical framework to quantify the significance of step-level and path-level calibrations in the context of Large Language Models (LLMs). 

(1) \emph{If step-level {\classB} is more significant than path-level one in the score $D_i$}, we can denote it as: 
$\forall n_j, n_k \in [1, N] ~ \text{and} ~ m_j, m_k \in [0, N], \text{where} ~ n_j < n_k ~ \text{and} ~ m_j > m_k$, the scores $D_j$ and $D_k$ should satisfy 
$$
\alpha \frac{n_j}{N} + (1 - \alpha) \frac{m_j}{M} > \alpha \frac{n_k}{N} + (1 - \alpha) \frac{m_k}{M} 
\label{eq:measure_score_sv_sc} 
$$
Thus we can obtain  
\begin{equation}
\alpha <  \frac{1} { \frac{ M(n_k-n_j) }{ N(m_j-m_k)} + 1 } 
\label{eq:measure_score_sv_sc_alpha}
\end{equation}
% \alpha < \frac{ N(m_j-m_k) }{ M(n_k-n_j) + N(m_j-m_k) }

If Eq~\eqref{eq:measure_score_sv_sc_alpha} is constant, we can infer that 
\begin{equation}
\alpha < \min \left( \frac{1} { \frac{ M(n_k-n_j) }{ N(m_j-m_k)} + 1 } \right)
 = \frac{1} { \frac{ M \max(n_k-n_j) }{ N \min(m_j-m_k)} + 1 }
\label{eq:measure_score_sv_sc_alpha_min}
\end{equation}
As $1 \leq n_j < n_k$, $n_j + n_k \leq N$, and $0 \leq m_k < m_j$, we can deduce that $\min(m_j - m_k) = 1$, $\max(n_k - n_j) = N - 2$. % = (N - 1) - 1
From the above, we deduce: 
\begin{equation}
\alpha < \frac{1}{ \frac{M(N-2)}{N} + 1 }
\label{eq:measure_score_sv_sc_alpha_min_final}
\end{equation} 
% $\min(m_j - m_k) = 1$, $\max(m_j - m_k) = M$; $\min(n_k - n_j) = 1$, $\max(n_k - n_j) = N - 2$
% Thus $\max \left( \frac{n_k-n_j}{m_j-m_k} \right) = \frac{\max(n_k - n_j)}{\min(m_j - m_k} = N - 2$. 

% Conversely, 
(2) \emph{If path-level {\classB} is more significant than step-level one in the score $D_i$}, we can denote it as: 
$\forall n_j, n_k \in [1, N] ~ \text{and} ~ m_j, m_k \in [0, N], \text{where} ~ n_j > n_k ~ \text{and} ~ m_j < m_k$, the scores $D_j$ and $D_k$ should also satisfy 
$$
\alpha \frac{n_j}{N} + (1 - \alpha) \frac{m_j}{M} > \alpha \frac{n_k}{N} + (1 - \alpha) \frac{m_k}{M} 
$$
Analogously, we can obtain 
\begin{equation}
\alpha >  \frac{1} { \frac{ M(n_j-n_k) }{ N(m_k-m_j)} + 1 } 
\label{eq:measure_score_sc_sv_alpha}
\end{equation}
If Eq~\eqref{eq:measure_score_sc_sv_alpha} is constant, we can infer that 
\begin{equation}
\alpha > \max \left( \frac{1} { \frac{ M(n_j-n_k) }{ N(m_k-m_j)} + 1 } \right) 
= \frac{1} { \frac{ M \min(n_j-n_k) }{ N \max(m_k-m_j)} + 1 } \
\label{eq:measure_score_sc_sv_alpha_max}
\end{equation}
As $1 \leq n_k < n_j$, $n_j + n_k \leq N$, and $0 \leq m_j < m_k$, we deduce that $\min(n_j - n_k) = 1$, $\max(m_k - m_j) = M - 0 = M$. 
From the above, we deduce: 
\begin{equation}
\alpha > \frac{1}{ \frac{1}{N} + 1}
\label{eq:measure_score_sc_sv_alpha_max_final}
\end{equation}


% Calculation of \texttt{ROSCOE} Scores.
\subsection{Evaluation of Answer Calibration} 
\label{sec:ROSCOE}
Calculation of \texttt{ROSCOE} Scores. Except for the classical evaluation metric, Accuracy, \citet{ICLR2023_ROSCOE} have proposed \textbf{\texttt{ROSCOE}}, a suite of metrics for multi-step reasoning, under four perspectives: 
semantic alignment (\texttt{ROSCOE-SA}), 
semantic similarity (\texttt{ROSCOE-SS}), 
logical inference, and (\texttt{ROSCOE-LI}) and 
language coherence (\texttt{ROSCOE-LC}). 
We select some scores from \texttt{ROSCOE} to do evaluation in our paper for space limits. Furthermore, these scores also show difference among various methods.  
% % fine-grained

Given source ground rationale ($\bm{s}$) and hypothesis generated rationale ($\bm{h}$) with multiple steps ($h_i$), we calculate five scores (\emph{All scores satisfy the principle that larger is better}): 

(1) Faithfulness$_{step}$ ($\bm{h} \rightarrow \bm{s}$): 
% To measure if the model misinterpreted the problem statement, or the reasoning path is too vague, irrelevant, or misuses information. 
To assess whether the model misconstrued the problem statement, or if the reasoning path is too nebulous, irrelevant, or improperly employs input information.
\begin{equation}
\textstyle\sum_{i=1}^{N}r\textnormal{-align}(h_i \rightarrow \bm{s}) / N 
\label{eq:faithfulness_step}
\end{equation}
where $N$ is the step number and $r\textnormal{-align}$ denotes reasoning alignment score. 
% To measure alignment from the hypothesis steps to the source sentences, by calculating the mean reasoning alignment score over the steps of reasoning。 

(2) Informativeness$_{path}$ ($\bm{h} \rightarrow \bm{s}$): 
To measure the level of concordance between the hypothesis path and the source, and if the generated reasoning path is well-grounded with respect to the source. 
% To quantify the degree of agreement between the hypothesis path and the source
\begin{equation}
[1 + \cos(\bm{h}, \bm{s})] / 2 
\label{eq:infor_path}
\end{equation} 

(3) Consistency$_{steps}$ ($h_i \leftrightarrow h_j$): 
To measure logical entailment errors \emph{within} the reasoning steps. 
\begin{equation}
1-\textstyle\max_{i=2..N} \textstyle\max_{j<i}p_{\mathrm{contr}}(h_i , h_j) 
\label{eq:consistency_step}
\end{equation} 
where $p_{\mathrm{contr}}$ is used to assess the likelihood of step pairs contradicting each other. 

(4) Consistency$_{path}$ ($\bm{h} \leftrightarrow \bm{s}$): 
To evaluate mistakes in logical entailment between the generated reasoning path $\bm{h}$ and source context $\bm{s}$: 
\begin{equation}
1 - \textstyle\max_{i=1..N} \textstyle\max_{j=1..T} ~p_{\mathrm{contr}}(h_i , s_j)
\label{eq:consistency_path}
\end{equation} 
where $p_{\mathrm{contr}}$ denotes the likelihood of source and hypothesis steps contradicting each other. 

(5) Perplexity$_{path}$ ($\bm{h}$): 
To calculate average perplexity of all tokens in the generated reasoning path steps. 
\begin{equation}
1 / \text{PPL}(\bm{h}) 
\label{eq:perplexity_path}
\end{equation} 
where $\text{PPL}$ denotes the perplexity. 
% The context used to score each token is the previous tokens in the current and all previous steps. Steps are joined with a space character. To keep the range and orientation consistent with the other scores we invert the perplexity. 


